A Framework to Prevent Biometric Data Leakage in the Immersive Technologies Domain

Doubtlessly, the immersive technologies have potential to ease people's life and uplift economy, however the obvious data privacy risks cannot be ignored. For example, a participant wears a 3D headset device which detects participant's head motion to track the pose of participant's head to match the orientation of camera with participant's eyes positions in the real-world. In a preliminary study, researchers have proved that the voice command features on such headsets could lead to major privacy leakages. By analyzing the facial dynamics captured with the motion sensors, the headsets suffer security vulnerabilities revealing a user's sensitive speech without user's consent. The psychography data (such as voice command features, facial dynamics, etc.) is sensitive data and it should not be leaked out of the device without users consent else it is a privacy breach. To the best of our literature review, the work done in this particular research problem is very limited. Motivated from this, we develop a simple technical framework to mitigate sensitive data (or biometric data) privacy leaks in immersive technology domain. The performance evaluation is conducted in a robust way using six data sets, to show that the proposed solution is effective and feasible to prevent this issue.

==> subsections/2-filter-algorithm.tex <==
\begin{table}
	\label{tab:freq}
	\begin{tabular}{l}
		\midrule
		\textbf{Algorithm 3:} The Proposed Filter Algorithm\\
		\midrule
		% \textbf{Phase 1:} \\
		\textbf{Input:}  \  \textit class\\
            % \ \ \  \ \ \ \ \ \ \  \textit $ \theta_D $ ( Features of the dataset ) \\
            \ \ \  \ \ \ \ \ \ \  $ \textit{D}_k \ (k = \{ \text{ECG, EEG, B-MOV,  UNKNOWN} \}) $ \\

            % \ \ \  \ \ \ \ \ \ \  \textit{Q} (set of audio signals)\\
            % \ \ \  \ \ \ \ \ \ \  \textit{$g_k(t)$} ( Signals for $t \geq t^*$, where $k \in P \cup Q$ )\\

           \textbf{if} $class == UNKNOWN $: \\
              \ \ \ \ \ \ \ \ \ \ allowed\_to\_pass = \textbf{TRUE} \\
            \textbf{else} \\
              \ \ \ \ \ \ \ \ \ \ allowed\_to\_pass = \textbf{FALSE} \\
            
            \\
            \textbf{Outcome:} \textit{allowed\_to\_pass} \\

		\bottomrule
	\end{tabular}
\label{algo:filter}
\end{table}


==> subsections/3-ProposedApproach.tex <==
\section{The Proposed Approach}

\input{AML/Images/architecture}

\input{AML/subsections/2-algorithm}
\input{AML/subsections/2-classifier-algorithm}
% \input{AML/subsections/2-filter-algorithm}

In this study, individual signals were collected separately from various datasets with a minimum duration of 8 seconds, adjusting the number of samples for the varying sample rates of the datasets. The overall algorithm is presented in Algorithm 1
The proposed approach consists of 3 main components.
\begin{enumerate}

    \item \textbf {Feature Extractor} - { In the existing literature, various features have been systematically collected to characterize different types of signals. For instance, in the context of a universal and privacy-preserving EEG-based authentication system, proposed methods include Autoregressive Models, Power Spectral Density analysis, and the utilization of Wavelet Transform for EEG signal  \cite{ Towards-privacy-EEG }.Similarly, in the case of Stable EEG Biometrics Using Convolutional Neural Networks and Functional Connectivity, models incorporating Power Spectral Density functions and fuzzy entropy measures are employed. Furthermore, Affective EEG-Based Person Identification, utilizing deep learning techniques, relies on Power Spectral Density estimation through Welch methods for individual identification based on EEG data \cite{Affective-EEG-Based}.\\
    Entropy-based methodologies have gained substantial recognition in characterizing physiological signals, spanning EEG, ECG, and blood pressure recordings. Notably, various studies have applied fuzzy entropy metrics for signal analysis and comparison purposes \cite{Fuzzy_Entropy_Metrics}. In addition, some research papers have incorporated distinctive features like PR and RR intervals for authentication objectives.\\
    In another context, studies has predominantly utilized spectral features, including spectral entropy, rolloff, and spread, alongside time-domain features such as energy metrics to authenticate individuals using head movements  \cite{head_authentication}. In our research, we adopted features that are common to ECG, EEG, and body movement signals, encompassing fuzzy entropy calculations spanning dimensions from 1 to 10, as well as statistical attributes of Power Spectral Density such as mean and standard deviation. These feature selections were made with a focus on robustness and universality across signal types.\\
    
    \item \textbf{Classifier}-  The extracted features served as the basis for training various machine learning models, encompassing Random Forest \cite{random-forest}, XGBoost \cite{xg-boost}, and LightGBM \cite{lightgbm}. Given the notable performance achieved by these individual models on the test data, there was no imperative need to pursue an ensemble of models. It is noteworthy that both XGBoost and LightGBM inherently exhibit ensemble characteristics, making the pursuit of additional ensemble strategies redundant in this particular context. \\
    To assess the robustness of the models under real-world conditions, various signal distortions were introduced. These distortions encompassed horizontal and vertical scaling, additive white Gaussian noise, and the use of smaller signal segments compared to the segments used for model training. Furthermore, superimposition of signals on audio was employed to simulate scenarios that could occur during signal transport or storage. Subsequently, the classification accuracy was used  to evaluate the performance of these models.
    \item \textbf{Filter}- Signal passage is determined by the classifier's probability prediction. If the classifier identifies the signals as ECG, EEG, or body movement data, they are barred from progression. The algorithm of the classifier and the filter is presented under Algorithm 2.
\end{enumerate}
. 



